FNAL PIP-II Accumulator Ring

The FNAL accelerator complex is poised to reach MW neutrino beams on target for the exploration of the dark sector physics and rare physics program spaces. Future operations of the complex will include CW linac operations at beam intensities that have not been seen before \cite{PIP2,RCS_LOI}. The ambitious beam program relies on multi-turn H$^{-}$ injection into the FNAL Booster and then extracted into delivery rings or the Booster Neutrino Beam (BNB) 8 GeV HEP program. A new rapid-cycling synchrotron (RCS) will be required to reach the LBNF goal of 2.4 MW because of intense space-charge limitations. There are many accelerator engineering challenges that are already known and many that will be discovered. This proposal calls for an intermediate step that will both facilitate the operation of Booster in the PIP-II era and gain operational experience associated with high power injection rings. This step includes the design, construction and installation of a 0.8 GeV accumulator ring (upgradeable to 1+ GeV) to be located in the PIP-II Booster Transfer Line (BTL). The PIP-II accumulator ring (PAR) may be primarily designed around permanent magnets or use standard iron core magnet technology with an aperture selected to accommodate the desired high intensity protons at 0.8 GeV.

==> chapters/RF.tex <==
\section{Storage Ring RF}

{\bf Timeline for all major activities and deliverables.}\\


